Diagnostic diagrams for ram-pressure stripped candidates

This paper presents a method for finding ram-pressure stripped (RPS) galaxy candidates by performing a morphological analysis of galaxy images obtained from the Legacy survey. We consider a sample of about 600 galaxies located in different environments such as groups and clusters, tidally interacting pairs and the field. The sample includes 160 RPS previously classified in the literature into classes from J1 to J5, based on the increasing level of disturbances. Our morphological analysis was done using the {\sc astromorphlib} software followed by the inspection of diagnostic diagrams involving combinations of different parameters like the asymmetry ($A$), concentration ($C$), S\'ersic index ($n$), and bulge strength parameters $F(G,\,M_{20})$. We found that some of those diagrams display a distinct region in which galaxies classified as J3, J4 and J5 decouples from isolated galaxies. We call this region as the morphological transition zone and we also found that tidally interacting galaxies in pairs are predominant within this zone. Nevertheless, after visually inspecting the objects in the morphological transition zone to discard obvious contaminants, we ended up with 33 bonafide new RPS candidates in the studied nearby groups and clusters (Hydra, Fornax, and CLoGS sample), of which one-third show clear evidence of unwinding arms. Future works may potentially further increase significantly the samples of known RPS using such method.

==> apendice.tex <==

\appendix

\section{{\bf Extended Table  of galaxies in the morphological transition zone}.}

\begin{table*}
\caption{Galaxies in the morphological transition zones}
\label{tab:Jelly_cand2}
\begin{tabular}{llccllcccccc}
\hline
\noalign{\smallskip}
Galaxy  & Cluster &RA & DEC  &   Morph  & $A$  & $C$  
  & $n$  &  $F(G,\,M_{20})$   &  intec  &  sep \\
  &  &[deg] & [deg]  &  &  &  &   
  &   &  & [kpc] \\
\hline
\noalign{\smallskip}
2MASX\,J01223182+0916534 &  LGG\,23	(CLoGS) & 20.6326  & 9.2815   & Early\_Tidal	     & 0.08 & 3.86  & 1.6   & 0.44  & -      & - \\
2MASX\,J10284923-3129509 &  Hydra	 & 157.2051 & -31.4975 & Early\_Blue\_Tidal  & 0.41 & 1.99  & 0.5   & -1.18 & -      & - \\
%2MASX\,J13280572-2925304 &  LGC\,351	 & 202.0240 & -29.4250 & Early\_Tidal	     & 0.01 & 4.06  & 2.5   & 0.57  & -      & - \\
2dFGRS\,TGS471Z004       &  Fornax	 & 49.8540  & -32.6493 & Irr  	     & 0.32 & 2.15  & 0.3   & -1.06 & -      & - \\
6dFGS\,gJ102734.0-234711 &  Hydra	 & 156.8911 & -23.7857 & Jelly  	     & 0.22 & 2.80  & 0.7   & -0.38 & Major  & 51.6 \\
6dFGS\,gJ103502.9-293024 &  Hydra	 & 158.7620 & -29.5066 & Early\_Blue\_Tidal  & 0.08 & 3.71  & 1.6   & 0.38  & -      & - \\
6dFGS\,gJ103704.4-312157 &  Hydra	 & 159.2685 & -31.3659 & Early\_Blue\_Tidal  & 0.19 & 3.10  & 1.0   & 0.04  & -      & - \\
%6dFGS\,gJ104139.4-274638 &  Hydra	 & 160.4143 & -27.7773 & Jelly  	     & 0.33 & 2.73  & 0.7   & -0.55 & -      & - \\
ESO\,302-14              &  Fornax	 & 57.9204  & -38.4522 & Jelly  	     & 0.29 & 2.20  & 0.8   & -0.92 & -      & - \\
ESO\,436-29		 &  Hydra    & 157.597    & -30.393    & Jelly & 0.35 & 2.2 & 0.4 & -0.80 & -  & - \\
ESO\,437-043 &   Hydra & 160.414 & -27.777 & Jelly & 0.33 & 2.7 & 0.7 & -0.55 & -  & - \\
ESO\,437-30		 &  Hydra	 & 159.812    & -30.298    & Spiral\_Edge-on & 0.25 & 3.6 & 0.8 & 0.20 & -  & - \\

ESO\,437-35		 &  Hydra	 & 160.018    & -30.267    & Spiral\_Egde-on & 0.31 & 2.7 & 0.4 & -0.88 & -  & - \\
ESO\,437-37		 &  Hydra	 & 160.129    & -29.270    & Jelly & 0.20 & 3.1 & 1.0 & 0.02 & -  & - \\
ESO\,437-50		 &  Hydra	 & 160.879    & -30.772    & Spiral\_SF & 0.31 & 2.7 & 0.6 & -0.65 & Major  & 34.0 \\
ESO\,437-64		 &  Hydra	 & 162.273    & -29.375    & Jelly & 0.28 & 3.0 & 0.9 & -0.42 & -  & - \\
ESO\,444-12		 &  LGG\,351 (CLoGS)	 & 200.209    & -29.480    & Jelly & 0.14 & 3.2 & 1.0 & 0.21 & -  & - \\
ESO\,500-42		 &  Hydra	 & 156.834    & -23.805    & Jelly & 0.23 & 3.8 & 1.2 & 0.42 & Major  & 50.8 \\
ESO\,501-22		 &  Hydra	 & 158.840    & -27.696    & Jelly & 0.22 & 3.1 & 0.6 & -0.21 & -  & - \\
ESO\,501-32		 &  Hydra	 & 159.092    & -25.377    & Spiral\_Tidal & 0.28 & 2.6 & 0.6 & -0.49 & -  & - \\
ESO\,501-61		 &  Hydra	 & 159.524    & -25.094    & Early\_Blue\_Tidal & 0.37 & 2.3 & 0.8 & -0.82 & -  & - \\
ESO\,501-65		 &  Hydra	 & 159.639    & -27.737    & Jelly & 0.42 & 2.7 & 0.7 & -0.50 & -  & - \\

ESO\,501-74		 &  Hydra	 & 160.205    & -24.668    & Jelly & 0.37 & 2.2 & 0.3 & -0.93 & -  & - \\
ESO\,501-9		 &  Hydra	 & 158.242    & -27.670    & Jelly & 0.29 & 2.4 & 0.4 & -1.14 & -  & - \\
ESO\,501-96		 &  Hydra	 & 161.698    & -23.328    & Early\_Blue\_Tidal & 0.13 & 3.4 & 1.5 & 0.19 & -  & - \\
%ESO\,507-21		 & LGG\,310	 & 192.619    & -26.843    & Early\_Tidal & 0.01 & 4.5 & 2.3 & 0.81 & -  & - \\
ESO\,507-28		 & LGG\,310	(CLoGS) & 192.941    & -26.090    & Jelly & 0.09 & 3.6 & 1.1 & 0.48 & Minor  & 29.2  \\
ESO\,507-35		 & LGG\,310 (CLoGS)     & 193.234    & -26.697    & Spiral\_Tidal & 0.24 & 2.5 & 1.0 & -0.73 & -  & - \\
ESO\,507-42		 & LGG\,310 (CLoGS)     & 193.400    & -26.294    & Spiral\_Edge-on & 0.15 & 3.5 & 1.2 & 0.27 & -  & - \\
ESO\,507-62		 & LGG\,310 (CLoGS)     & 194.846    & -27.427    & Spiral\_Edge-on & 0.25 & 2.7 & 0.6 & -0.58 & -  & - \\
IC\,401 		 & LGG\,126  (CLoGS)    &  76.082    & -10.077    & Spiral\_Edge-on & 0.50 & 3.6 & 1.0 & 0.05 & -  & - \\	   
%IC\,1797		 & LGG\,61       &  36.366    & 20.395     & Spiral\_Edge-on & 0.21 & 3.9 & 1.7 & 0.85 & -  & - \\	   
IC\,2537		 & LGG\,185 (CLoGS)      &  150.966   & -27.571    & Jelly & 0.27 & 2.5 & 0.4 & -0.72 & -  & - \\		   
IC\,4248		 & LGG\,351	(CLoGS) &  201.697   & -29.881    & Jelly & 0.37 & 3.6 & 0.7 & 0.03 & -  & - \\		   


IC\,4275		 & LGG\,351	(CLoGS) &  202.964   & -29.732    & Jelly & 0.24 & 2.5 & 0.7 & -0.78 & -  & - \\		   
IC\,4397		 & LGG\,383  (CLoGS)    &  214.495   & 26.413     & Jelly & 0.30 & 3.1 & 0.6 & -0.21 & -  & - \\		   
LEDA\,722049		 & Hydra	 &  160.790   & -30.050    & Spiral\_SF & 0.28 & 2.8 & 1.0 & -0.45 & -  & - \\	   
LEDA\,753354		 & Hydra	 &  159.343   & -27.545    & Jelly & 0.47 & 1.8 & 0.2 & -0.94 & INDEF  & 31.0 \\	   
MCG-01-10-036		 & LGG\,103 (CLoGS)     &  56.741    & -3.462     & Jelly & 0.25 & 3.4 & 0.6 & 0.06 & -  & - \\		   
MCG-03-34-014		 & LGG\,338	(CLoGS) &  198.148   & -17.542	   & Spiral\_Edge-on & 0.23 & 2.9 & 0.5 & -0.79 & -  & - \\	 
MCG-04-25-054		 & Hydra	 &  159.858   & -23.755	   & Jelly & 0.24 & 3.6 & 0.7 & 0.11 & -  & - \\  		 
ESO\,500-14          & Hydra     & 156.131    & -23.553    & Early\_Tidal & 0.18 & 2.9 & 0.9 & -0.27 & -  & - \\
%NGC\,374                 & LGG\,18	 & 16.774     & 32.795     & Early\_Tidal & 0.02 & 4.3 & 1.8 & 0.37 & -  & - \\
%NGC\,399 		 & LGG\,18	 & 17.247     & 32.634     & Early\_Tidal & 0.04 & 4.4 & 2.1 & 0.62 & -  & - \\
%NGC\,420 		 & LGG\,18	 & 18.040     & 32.123     & Early\_Tidal & 0.04 & 4.5 & 2.0 & 0.88 & -  & - \\
NGC\,489 		 & LGG\,23 (CLoGS)	 & 20.475     & 9.207	   & Spiral\_Edge-on & 0.09 & 3.6 & 1.1 & 0.35 & -  & - \\
%NGC\,502 		 & LGG\,23	 & 20.731     & 9.049	   & Early\_Tidal & 0.01 & 4.0 & 2.2 & 0.39 & -  & - \\
NGC\,518 		 & LGG\,23 (CLoGS)	 & 21.068     & 9.325	   & Early\_Edge-on & 0.22 & 3.5 & 0.9 & 0.08 & -  & - \\

NGC\,586 		 & LGG\,27 (CLoGS)	 & 22.904     & -6.894     & Early\_Edge-on & 0.16 & 3.6 & 1.2 & 0.35 & Minor  & 37.1 \\
NGC\,600 		 & LGG\,27 (CLoGS)      & 23.272     & -7.312     & Spiral\_SF & 0.21 & 2.6 & 0.4 & -0.23 & -  & - \\
%NGC\,615 		 & LGG\,27	 & 23.774     & -7.340     & Spiral\_Edge-on & 0.15 & 4.4 & 1.4 & 0.80 & -  & - \\
%NGC\,924 		 & LGG\,61       & 36.695     & 20.498     & Spiral\_Edge-on & 0.06 & 4.7 & 2.3 & 0.85 & -  & - \\
NGC\,1341		 & Fornax     & 51.992     & -37.149    & Spiral\_Tidal & 0.28 & 2.7 & 0.9 & -0.48 & -  & - \\
NGC\,1376		 & LGG\,103 (CLoGS)      & 54.273     & -5.044     & Jelly & 0.35 & 2.6 & 0.5 & -0.66 & -  & - \\
%NGC\,1386		 & Fornax	 & 54.192     & -35.999    & Early\_Edge-on & 0.17 & 4.4 & 0.9 & 0.67 & INDEF  & 41.3 \\
NGC\,1417		 & LGG\,103 (CLoGS)     & 55.489     & -4.705     & Spiral\_Tidal & 0.24 & 3.5 & 0.8 & 0.02 & -  & - \\
NGC\,1418		 & LGG\,103 (CLoGS)     & 55.567     & -4.731     & Jelly & 0.30 & 2.7 & 0.5 & -0.73 & -  & - \\
%NGC\,1441		 & LGG\,103  	 & 56.430     & -4.092     & Early\_Edge-on & 0.13 & 3.9 & 1.6 & 0.62 & -  & - \\
NGC\,1449		 & LGG\,103 (CLoGS)      & 56.513     & -4.138     & Early\_Tidal & 0.02 & 3.9 & 1.8 & 0.47 & -  & - \\
%NGC\,1451		 & LGG\,103      & 56.530     & -4.069     & Early\_Tidal & 0.01 & 3.7 & 2.1 & 0.38 & -  & - \\
%NGC\,2911		 & LGG\,177	 & 143.442    & 10.153     & Early\_Tidal & 0.21 & 4.3 & 1.8 & 0.46 & -  & - \\
%NGC\,2914		 & LGG\,177	 & 143.512    & 10.109      & Early\_Tidal & 0.06 & 3.6 & 2.1 & 0.74 & INDEF  & 52.1 \\
NGC\,2939	         & LGG\,127	(CLoGS)  & 144.533 & 9.524   & Jelly & 0.47 & 2.9 & 0.8 & 0.08 & -  & - \\
%NGC\,3314		 & Hydra	  & 159.304 & -27.684  & Jelly & 0.33 & 2.7 & 0.6 & -0.59 & -  & - \\
NGC\,3383		 & Hydra	  & 161.830 & -24.438  & Spiral\_SF & 0.25 & 2.5 & 0.6 & -0.80 & -  & - \\
NGC\,3625		 & LGG\,232	(CLoGS)  & 170.130 & 57.781  & Spiral\_Edge-on & 0.19 & 2.8 & 0.7 & -0.12 & -  & - \\
%NGC\,3648		 & LGG\,236	  & 170.631 & 39.877  & Early\_Tidal & 0.01 & 4.2 & 1.8 & 0.54 & -  & - \\
NGC\,3652		 & LGG\,236	(CLoGS)  & 170.663 & 37.765  & Spiral\_Tidal & 0.50 & 2.4 & 0.4 & -0.38 & -  & - \\
NGC\,3669		 & LGG\,232 (CLoGS) 	  & 171.362 & 57.721  & Spiral\_Edge-on & 0.21 & 2.9 & 0.4 & -0.95 & -  & - \\
%NGC\,5150		 & LGG\,351	  & 201.902 & -29.562 & Spiral\_Tidal & 0.08 & 4.4 & 2.1 & 0.79 & -  & - \\
%NGC\,5342		 & LGG\,360	  & 207.858 & 59.864 & Early\_Tidal & 0.01 & 4.0 & 1.9 & 0.54 & -  & - \\
%NGC\,5389		 & LGG\,360	  & 209.026 & 59.742 & Early\_Edge-on & 0.31 & 4.4 & 1.8 & 0.72 & Major  & 33.4 \\
NGC\,5635		 & LGG\,383	(CLoGS)  & 217.132 & 27.409 & Jelly & 0.28 & 3.9 & 1.1 & 0.15 & -  & - \\
NGC\,5653		 & LGG\,383	(CLoGS)  & 217.543 & 31.215 & Early\_Tidal & 0.27 & 2.9 & 1.3 & 0.01 & -  & - \\
%NGC\,5657		 & LGG\,383	  & 217.682 & 29.181 & Spiral\_Edge-on & 0.13 & 4.1 & 1.5 & 0.73 & -  & - \\
NGC\,5735		 & LGG\,383	(CLoGS)  & 220.639 & 28.726 & Jelly & 0.33 & 2.6 & 0.6 & -0.44 & -  & - \\
NGC\,5989		 & LGG\,402	(CLoGS)  & 235.387 & 59.755 & Jelly & 0.29 & 2.2 & 0.5 & -0.93 & -  & - \\
NGC\,1427A		 & Fornax	  & 55.038 & -35.626  & Jelly & 0.41 & 2.3 & 0.4 & -0.80 & INDEF  & 47.9 \\
NGC\,1437A		 & Fornax	  & 55.758 & -36.273  & Jelly & 0.39 & 2.5 & 0.4 & -0.55 & -  & - \\
NGC\,3314A & Fornax & 159.304 & -27.684 &  Jelly & 0.33 & 2.7 & 0.6 & -0.59 & -  & - \\
UGC\,724		 & LGG\,18	  & 17.498 & 32.368 & Jelly & 0.08 & 3.4 & 1.6 & 0.31 & -  & - \\
\noalign{\smallskip} 
\hline
\noalign{\smallskip}

\end{tabular}
\end{table*}


\begin{table*}
\contcaption{Galaxies in the jellyfish zone}
\begin{tabular}{llccllcccccc}
\hline
\noalign{\smallskip}
Galaxy  & Cluster &RA & DEC  &   Morph  & $A$  & $C$  
  & $n$  &  $F(G,\,M_{20})$   &  intec  &  sep \\
  &  &[deg] & [deg]  & &  &  &  
  &   &  & [kpc] \\
\hline
\noalign{\smallskip}
UGC\,743		 & LGG\,18	(CLoGS)  & 17.827 & 31.889 & Early\_Tidal & 0.11 & 3.4 & 1.2 & 0.24 & -  & - \\
UGC\,803		 & LGG\,23 (CLoGS)       & 18.845 & 8.099  & LBS & 0.26 & 2.9 & 1.4 & -0.52 & -  & - \\
UGC\,1980		 & LGG\,66	(CLoGS)  & 37.640 & 32.176 & Spiral\_Edge-on & 0.21 & 3.0 & 0.8 & -0.02 & -  & - \\
UGC\,2032		 & LGG\,61	(CLoGS)  & 38.352 & 20.579 & Spiral\_Edge-on & 0.14 & 3.5 & 0.6 & 0.05 & -  & - \\
UGC\,6433		 & LGG\,236	(CLoGS)  & 171.383 & 38.061 & Early\_Blue\_Tidal & 0.40 & 3.0 & 0.7 & -0.68 & -  & - \\
UGC\,8199		 & LGG\,329 (CLoGS)       & 196.688 & 35.101 & Jelly & 0.27 & 2.6 & 0.6 & -0.69 & Major  & 59.9 \\
UGC\,8200		 & LGG\,329	(CLoGS)  & 196.733 & 35.132 & Jelly & 0.36 & 2.9 & 0.7 & -0.18 & Major  & 57.8 \\
UGC\,9253		 & LGG\,383	(CLoGS)  & 216.744 & 31.517 & Spiral\_Edge-on & 0.19 & 3.2 & 0.5 & -0.15 & -  & - \\
UGC\,9302		 & LGG\,383 (CLoGS)       & 217.291 & 31.799 & Jelly & 0.25 & 3.4 & 0.6 & -0.26 & -  & - \\
WPVS\,78		 & Hydra	  & 159.672 & -25.592& Spiral\_Tidal & 0.41 & 2.1 & 0.8 & -0.84 & -  & - \\

\noalign{\smallskip} 
\hline
\noalign{\smallskip}

\end{tabular}
\end{table*}


\section{Residual images of the RPS candidates.}

\begin{figure*}
\centering
\includegraphics*[width=0.45\textwidth]{figures/fig_6dFGSgJ102734.0-234711_model.png}
\includegraphics*[width=0.45\textwidth]{figures/fig_ESO302-14_model.png}
\includegraphics*[width=0.45\textwidth]{figures/fig_ESO436-29_model.png}
\includegraphics*[width=0.45\textwidth]{figures/fig_ESO437-043_model.png}
\includegraphics*[width=0.45\textwidth]{figures/fig_ESO437-37_model.png}
\includegraphics*[width=0.45\textwidth]{figures/fig_ESO437-64_model.png}
\includegraphics*[width=0.45\textwidth]{figures/fig_ESO444-12_model.png}
\includegraphics*[width=0.45\textwidth]{figures/fig_ESO500-42_model.png}
\includegraphics*[width=0.45\textwidth]{figures/fig_ESO501-74_model.png}
\includegraphics*[width=0.45\textwidth]{figures/fig_ESO501-9_model.png}
\caption{Residual images of the RPS candidates. Each column contains the input image (left) and residual image
{\bf in $g$-band} (left) for each RPS candidate. The grey regions visible in the residual maps represent areas that have been intentionally masked during the analysis. These masks are applied to distinguish between various components in the data, such as segmentation maps for background galaxies and foreground stars. The North ($\delta$) and East ($\alpha$) directions are aligned in the conventional way.}
\label{fig_model_jelly_01}
\end{figure*}


\begin{figure*}
\contcaption{}
\includegraphics*[width=0.45\textwidth]{figures/fig_ESO507-28_model.png}
\includegraphics*[width=0.45\textwidth]{figures/fig_IC2537_model.png}
\includegraphics*[width=0.45\textwidth]{figures/fig_IC4275_model.png}
\includegraphics*[width=0.45\textwidth]{figures/fig_IC4397_model.png}
\includegraphics*[width=0.45\textwidth]{figures/fig_LEDA753354_model.png}
\includegraphics*[width=0.45\textwidth]{figures/fig_MCG-01-10-036_model.png}
\includegraphics*[width=0.45\textwidth]{figures/fig_MCG-04-25-054_model.png}
\includegraphics*[width=0.45\textwidth]{figures/fig_NGC1376_model.png}
\includegraphics*[width=0.45\textwidth]{figures/fig_NGC1418_model.png}
\includegraphics*[width=0.45\textwidth]{figures/fig_NGC2939_model.png}
\label{fig_model_jelly_02}
\end{figure*}


\begin{figure*}
\centering
\includegraphics*[width=0.45\textwidth]{figures/fig_NGC3314A_model.png}
\includegraphics*[width=0.45\textwidth]{figures/fig_NGC5735_model.png}
\includegraphics*[width=0.45\textwidth]{figures/fig_NGC5989_model.png}
\includegraphics*[width=0.45\textwidth]{figures/fig_NGC1427A_model.png}
\includegraphics*[width=0.45\textwidth]{figures/fig_NGC1437A_model.png}
\includegraphics*[width=0.45\textwidth]{figures/fig_UGC724_model.png}
\includegraphics*[width=0.45\textwidth]{figures/fig_UGC8199_model.png}
\includegraphics*[width=0.45\textwidth]{figures/fig_UGC8200_model.png}
\includegraphics*[width=0.45\textwidth]{figures/fig_UGC9302_model.png}
\contcaption{}
\label{fig_model_jelly_03}
\end{figure*}








\begin{figure*}
\centering
\includegraphics*[width=0.8\textwidth]{figures/fig_ESO436-29_rt.png}
\includegraphics*[width=0.8\textwidth]{figures/fig_ESO437-64_rt.png}
\includegraphics*[width=0.8\textwidth]{figures/fig_ESO501-65_rt.png}
\includegraphics*[width=0.8\textwidth]{figures/fig_IC2537_rt.png}
\caption{The unwinding ram pressure galaxy candidates. Left panels contain the deprojected images {\bf in the $g$-band}, while right panels contain the radius {\it vs} $\theta$ plots. The ``X'' 's are the markers for the spiral arms for which were measured the aperture angles, while the black arrows indicate
the inner and outer ranges for the arms. The North ($\delta$) and East ($\alpha$) directions are aligned in the conventional way.}
\label{fig_unwinding_01}
\end{figure*}


\begin{figure*}
\centering

\includegraphics*[width=0.8\textwidth]{figures/fig_IC4275_rt.png}
\includegraphics*[width=0.8\textwidth]{figures/fig_NGC1376_rt.png}
\includegraphics*[width=0.8\textwidth]{figures/fig_NGC1437A_rt.png}
\includegraphics*[width=0.8\textwidth]{figures/fig_NGC2939_rt.png}
\contcaption{}
\label{fig_unwinding_02}
\end{figure*}



\begin{figure*}
\centering
\includegraphics*[width=0.8\textwidth]{figures/fig_UGC724_rt.png}
\includegraphics*[width=0.8\textwidth]{figures/fig_UGC8200_rt.png}
\contcaption{}
\label{fig_unwinding_03}
\end{figure*}


%\begin{figure*}
%\centering
%\includegraphics*[width=0.45\textwidth]%{figures/fig_UGC8199_model.png}
%\includegraphics*[width=0.45\textwidth]{figures/fig_UGC8200_model.png}
%\includegraphics*[width=0.5\textwidth]{figures/fig_UGC9302_model.png}
%\contcaption{}
%\label{fig_model_jelly_04}
%\end{figure*}

%\begin{figure*}
%\centering
%\includegraphics*[angle=0,width=0.8\textwidth]{figures/fig_ESO 437-64_model.png}
%\includegraphics*[angle=0,width=0.8\textwidth]{figures/fig_ESO 444-12_model.png}
%\hspace*{-5pt}
%\includegraphics*[angle=0,width=0.8\textwidth]{figures/fig_ESO 500-42_model.png}
%\hspace*{-5pt}
%\includegraphics*[angle=0,width=0.8\textwidth]{figures/fig_ESO 501-9_model.png}
%\hspace*{-5pt}
%\includegraphics*[angle=0,width=0.8\textwidth]{figures/fig_ESO 501-22_model.png}
%\contcaption{}
%\label{fig_model_jelly_01}
%\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% End of mnras_template.tex

